A Web of Blocks

Blockchains offer a useful abstraction: a trustworthy, decentralized log of totally ordered transactions. Traditional blockchains have problems with scalability and efficiency, preventing their use for many applications. These limitations arise from the requirement that all participants agree on the total ordering of transactions. To address this fundamental shortcoming, we introduce Charlotte, a system for maintaining decentralized, authenticated data structures, including transaction logs. Each data structurestructure -- indeed, each block -- specifies its own availability and integrity properties, allowing Charlotte applications to retain the full benefits of permissioned or permissionless blockchains. In Charlotte, a block can be atomically appended to multiple logs, allowing applications to be interoperable when they want to, without inefficiently forcing all applications to share one big log. We call this open graph of interconnected blocks a blockweb. We allow new kinds of blockweb applications that operate beyond traditional chains. We demonstrate the viability of Charlotte applications with proof-of-concept servers running interoperable blockchains. Using performance data from our prototype, we estimate that when compared with traditional blockchains, Charlotte offers multiple orders of magnitude improvement in speed and energy efficiency.

==> Makefile <==
# DOC defines the version of the document being generated.
# It should be one of: markup, local, submission, final, finaldraft, tr, trdraft
# See paperversions.tex for the explanation of how the versions differ.
#
# Use 'make DOC' for appropriate values of DOC to build the corresponding document

DOC = draft
# Set DOC to one of draft, local, submission, final, finaldraft, report

# Name of the top-level TeX file sans .tex extension
CONF = paper

TARGETS = $(DOC).pdf

default: $(TARGETS)

TEXS = $(DOC).tex abstract.tex header.tex body.tex introduction.tex           \
    tableofcontentsparagraph.tex supplychain.tex                              \
    entanglement.tex design.tex                                               \
    attestations.tex life.tex chains.tex consistency.tex                      \
    causal.tex joins.tex chain.tex applications.tex simulating.tex            \
    object.tex application-supply.tex incentives.tex banking.tex              \
    disreputable.tex timestamping.tex version.tex medical.tex                 \
    evaluation.tex twoaccounts.tex implementation.tex                         \
    performance.tex discussion.tex extensions.tex confidentiality.tex         \
    deletion.tex compacting.tex conclusion.tex related.tex unchained.tex      \
    meets.tex structure.tex policies-availability.tex policies-integrity.tex  \
    labels.tex reference.tex chains-as-objects.tex blocks-as-transactions.tex \
    experimental.tex consensus.tex

# included figures
FIGS = fig-block.tex fig-reference.tex images/fern.pdf                        \
    images/wilburStorage.pdf fig-life.tex fig-twoaccounts.tex                 \
    fig-endorsement.tex images/block-B.pdf images/cloud-Blue.pdf              \
    images/cloud-Red.pdf images/ribbon-Blue.pdf images/ribbon-Red.pdf         \
    fig-evaluation.tex fig-chains.tex images/label-yellow.pdf                 \
    images/label-red.pdf images/label-green.pdf images/label-blue.pdf

# change to wherever commondefs is located
PAPERSROOT = ..
MAKEDIR = make

include $(MAKEDIR)/commondefs

# overrides to commondefs
TEXDIR = tex-macros
BIBFILE = bibtex/pm-master.bib

LDIRT = local.tex markup.tex draft.tex submission.tex final.tex               \
        finaldraft.tex tr.tex trdraft.tex blindtr.tex web.tex

GENERATED += local.* markup.* draft.* submission.* final.* finaldraft.* tr.*  \
             trdraft.* blindtr.* web.*

TEXINPUTS = acmart:tex-macros:

VPATH = acmart

LATEXFLAGS = -shell-escape

$(DOC).tex: $(CONF).tex
	sed s/DOC/$(DOC)/ < $(CONF).tex > $(DOC).tex
   
$(DOC).pdf: $(TEXS) $(FIGS) $(DOC).stamp $(DOC).bbl $(BIBFILE) acmart.cls

$(DOC).bbl: $(BIBFILE) $(DOC).stamp ACM-Reference-Format.bst

# rules to ensure submodules are present
acmart.cls ACM-Reference-Format.bst:
	git submodule update --init
	$(MAKE) -C acmart acmart.cls

$(BIBFILE):
	git submodule update --init

include $(COMMONRULES)


==> acmart/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	sample-manuscript.tex \
	sample-acmsmall.tex \
	sample-acmlarge.tex \
	sample-acmtog.tex \
	sample-sigconf.tex \
	sample-sigconf-authordraft.tex \
	sample-sigconf-xelatex.tex \
	sample-sigplan.tex \
	sample-sigchi.tex \
	sample-sigchi-a.tex


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

sample-sigconf-xelatex.pdf:  sample-sigconf-xelatex.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	xelatex $<
	- bibtex $*
	xelatex $<
	xelatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do xelatex $<; done

sample-manuscript.pdf \
sample-acmsmall.pdf \
sample-acmlarge.pdf \
sample-acmtog.pdf: samplebody-journals.tex

sample-sigconf.pdf \
sample-sigconf-authordraft.pdf \
sample-sigconf-xelatex.pdf \
sample-sigplan.pdf \
sample-sigchi.pdf: samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf sample-*.pdf *.cls *.bst


==> acmart/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.  


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
		Sigch-a sample bibliography renamed
		Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
		Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
		Corrected the bug with acmPrice.
		Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
		The package now is compatible with polyglossia (Joachim Breitner).
		Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

==> bitcoin.tex <==
The bitcoin payment network doesn't keep track of money in terms of
 accounts, the way our proposed Charlotte-based banking system
 would~\p{\autoref{sec:banking}}.
Instead, each transaction divides all its money into a number of
 outputs, each of which specify the conditions under which they can be
 spent (e.g. you need a signature matching this public key ...).
These are called Unspent Transaction Outputs, or UTXOs.
Each transaction specifies a set of input UTXOs as well, from whence
 it gets the money, and provides for each a proof that it is
 authorized to spend the money (e.g. a digital signature).
Each UTXO is completely drained when it is spent, and cannot be
 re-used.
Thus the transactions in Bitcoin form a graph, with transactions as
 vertices, and UTXOs as directed edges~\cite{bitcoin}.

In our Charlotte banking model, each bank account is a chain, and so
 transfers between two accounts are simply a block on both chains.
Therefore, so far as two sets of financial transactions don't
 interact, they can operate entirely in parallel.
The fundamental speed limiter of the whole system is the speed of the
 slowest chain.
If all transactions are between exactly two accounts, and it always
 takes the same amount of time to append a block to two chains, then
 this\ACM{indefinite reference} is simply the length of the longest chain.

In blocks \bitcoinstartblock{} through \bitcoinendblock{} of bitcoin,
 there are \bitcoinnumtransactions{} transactions.
The longest chain through this graph is \bitcoinlengthlongest{}, and
 so, in principle, charlotte needs time for only
 \bitcoinlengthlongest{} rounds of consensus to accommodate the entire
 payment graph.
Even though bitcoin batches several transactions per block, it
 required \bitcoinnumblocks{} rounds of consensus to do the same,
 taking a total of \bitcointotaltime{}.
Thus, even with a similarly slow consensus mechanism, Charlotte would
 require only \bitcoincharlottetotaltime{}.
Of course, Charlotte bank accounts can specify Fern servers with
 whatever consensus mechanism they like.
Presumably, this could be a much faster system, such as
 PBFT~\cite{pbft}.

In bitcoin, it is advantageous to combine many small transfers of
 money into big ones, with many inputs and many outputs.
This improves anonymity and performance.
In the real financial system of the USA, however, all monetary
 transfers are from one account to another.
They are all exactly two chain transactions.

We can simulate this limitation by refactoring each Bitcoin transaction
 as a DAG of transactions with depth:
\[
\left\lceil log_2\p{max\p{\textrm{number of inputs}, \textrm{ number of outputs}}} \right\rceil
\]
(See \autoref{sec:twoaccounts} for how.)

With this construction, Charlotte executes more than one transaction
 per bitcoin transaction.
The longest chain through this new transaction graph is
 \bitcoinlengthlongestweighted{}, and so, in principle, charlotte
 needs time for only \bitcoinlengthlongestweighted{} rounds of
 consensus to accommodate the entire payment graph.
Thus, even with a similarly slow consensus mechanism to bitcoin,
 Charlotte would still require only
 \bitcoincharlotteweightedtotaltime{}.
Even with our unoptimized proof-of-concept implementation, with each
 chain running a 4-participant byzantine-tolerant consensus amongst
 its Fern servers, we could append a block to two chains in
 $15.8\pm0.8$ seconds.
What took the bitcoin system \bitcointotaltime{} would thus take
 Charlotte \bitcoincharlotteweightedexperimenttime{}, a mere
 \bitcoincharlotteweightedexperimenttimepercent of bitcoin's time.
 


==> draft.tex <==
\def\paperversion{draft}
\def\anonymoussubmission{1} % remove or change to 0 to make submission non-anonymous
\input{paperversions}
\input{header}
\begin{document}
\input{body}
\end{document}


==> interoperability.tex <==
With current blockchain architectures, it is impossible to commit the
 same record to multiple blockchains.
Each chain has its own formatting and protocols, and there is no
 uniform way to even reference one chain from another.
As a result, applications on different chains cannot interact.
There is no simple way, for instance, to atomically commit a trade of
 Bitcoins for Ether to both the {\bitcoin} and {\ethereum}
 blockchains.
This is evidenced by the development of elaborate workarounds, such
 as the interledger protocol, which specifically handles
 cryptocurrency trades~\cite{interledger}.

In particular, three fundamental features dramatically improve
 cross-chain interoperability:
\begin{itemize}
\item \textit{References}: While all blockchains reference blocks by
 hash, different chains format their references differently.
Furthermore, it is not clear from a reference where the block can be
 found, or if it has been irrevocably committed to a data structure.
This feature may be the simplest, but most important.
\item \textit{Attestations}: Each block read must feature some proof
 that it will remain available, and that it is committed to any
 relevant data structures.
These attestations might include, say, a signed statement from a
 storage server (or even a proof of
 retrievability\ICS{citation needed}) vowing to store the block
Other examples include proofs of work, or records of consensus,
 demonstrating that conflicting blocks won't be allowed in a given
 data structure.
\item \textit{Atomic Commitments}: In records to be added atomically
 to two structures at once, the attestation satisfying both structures
 should be generated together, or not at all.
For instance, if \principalA{} wishes to trade \commodityA{} to
 \principalB{} in exchange for \commodityB{}, and there are separate
 authorities tracking \commodityA{} and \commodityB{}, then it would
 be bad if \principalB{} got the \commodityA{}, but \principalA{}
 didn't get the \commodityB{}.
\end{itemize}

Charlotte's block specification provides a format for each of these.
\ICS{Should this paragraph really be in this section?}
Our example implementation features references by SHA2 hash and
 storage attestations in the form of signed permanent promises to
 provide the block~\p{\autoref{sec:attestations}}.
Our chain data structures feature proofs of consensus vowing that the
 participants will not accept any other block in that slot on that
 chain~\p{\autoref{sec:chains}}.
Our atomic commits are made from \textit{meets} of
 consensus specifications: they consent together or not at
 all~\p{\autoref{sec:joins}}.


==> life.tex <==

Each block is minted by some client application.
The client constructs the block as a Merkle tree, with one leaf being
 a label~\p{\autoref{sec:labels}}.
Once the block is constructed, the client needs to gather Wilbur and
 Fern attestations to create a reference to the new block.
A timeline of this process is in~\autoref{fig:life}.

The client first stores the block on some Wilbur servers, and obtains
 from each an attestation, so that together, the attestations are
 sufficient to satisfy the availability policy of the label.
These attestations, along with the Merkle root of the block, the label
 of the block, and a Merkle proof that the label is a leaf of the
 root, are sent to Fern servers.
The Fern servers may produce integrity attestations.
If---perhaps because a conflicting block was already approved---the Fern
 servers cannot accept the block, they may inform the client as to why.
The reasons for block rejections, and the information Fern servers
 should send back to clients, are application-specific.
\RVR{RE: ``This is beyond the scope of the protocol.''
     The scope of this protocol as far as this paper is concerned?
     Do we need to say it?
}\ICSreply{Well, reasons for conflicts, and the explanations Fern
            servers send to clients, are application specific.
           I'm not certain that we need to say that, though.}

The label, root hash, Merkle proof,
 \RVR{Doesn't the Merkle proof include the Merkle root?
 }\ICSreply{Yes, and in fact in the reference format they're combined,
             but I wasn't sure if that would be immediately obvious to
             the reader, and it seems reasonable to explictly say that
             the root hash goes in the reference.}
 and attestations together form a
 block reference, which other blocks should use when referring to this
 one.
Fern servers may wish to store this reference where appropriate
 parties can find it (e.g. Wilbur servers, or the client).


\ICS{There is a chicken-and-egg problem here, which we might consider
 putting in the paper:
However, as the reference itself is essentially a unit of information,
 it cannot self-attest to its own availability, for the same reason
 blocks cannot.
The reference must exist before it can be stored, and stored before
 attestations of its storage can exist.
As other blocks may include this reference, the reference itself will
 be as available as those blocks.
}\ICSreply{The latter half of this paragraph is a bit of a downer.
     The reality is not so bad as this makes it seem.
     Since references will be found in other blocks, the availability
      of those blocks renders the references available.
     Basically, the limitation amounts to: 
      If you don't have a reference to a block, you can't be
      sure it exists.}
\RVRreply{Why not include this in the paper?
          The ``best-effort'' label is hard to understand.}
\ICSreply{well, for the moment, none of it is in the paper.}


==> make/commondefs <==
#
# See the manual page for "commondefs" for more information.
#

INCLDIR = $(ROOT)/usr/include
PAPERSROOT ?= ..
TEXDIR = $(PAPERSROOT)/tex-macros

COMMONRULES = $(MAKEDIR)/commonrules

SOURCES = $(CFILES) $(C++FILES) $(YFILES) $(LFILES) $(AFILES)
OBJECTS = $(CFILES:.c=.o) $(C++FILES:.C=.o)
DIRT = *.o core *.aux* *.dvi *.log *.stamp *.i *.bbl *.out *.upa *.upb *.[ib]lg $(LDIRT)
GENERATED = .dependtime Makedepend Makedepend.bak
RM = rm -f
MKDEPFILE = Makedepend
MKDEPEND = makedepend
MKDEPFLAGS = -Y
MKDEPC++FLAGS = $(C++DEFS) $(C++INCS) $(MKDEPFLAGS)
MKDEPCFLAGS = $(CDEFS) $(CINCS) $(MKDEPFLAGS)

.SUFFIXES: .C .ps .i .txt .h
.SUFFIXES: .tex .dvi .ind .idx .bbl .aux .glo .aux .stamp .pdf .eps

GNUBIN = /usr/local

ATTC++ = CC
DECC++ = cxx
GNUC++ = g++

CC = cc
C++ = $(GNUC++)
YACC = bison
DVIPS = dvips

C++F = $(C++) $(C++FLAGS)
CCF = $(CC) $(CFLAGS)

C++FLAGS = $(C++OPTS) $(C++DEFS) $(C++INCS)

C++INCS = $(GC++INCS) $(LC++INCS)
C++OPTS = $(GC++OPTS) $(LC++OPTS)
C++DEFS = $(GC++DEFS) $(LC++DEFS)

GC++OPTS = $(OPTIMIZER)

CFLAGS = $(COPTS) $(CDEFS) $(CINCS)
COPTS = $(GCOPTS) $(LCOPTS)
CDEFS = $(GCDEFS) $(LCDEFS)
CINCS = $(GCINCS) $(LCINCS)

GCOPTS = $(OPTIMIZER)

M3F = $(M3) $(M3FLAGS)
M3 = m3
M3PP = m3pp

LDFLAGS = $(LLDFLAGS) $(GLDFLAGS)
LLDFLAGS = $(LLDLIBS) $(LLDOPTS) 

SEP=:
#SEP=\;         # for MikTeX+Cygwin # Deprecated: define this in $(MAKEDIR)/localdefs
TEXINPUTS = .$(SEP)$(TEXDIR)$(SEP)
LATEX = TEXINPUTS='$(TEXINPUTS)' $(LATEXEXEC) $(LATEXFLAGS)
PDFLATEX = TEXINPUTS='$(TEXINPUTS)' $(PDFLATEXEXEC) $(PDFLATEXFLAGS)
LATEXEXEC = latex
PDFLATEXEXEC = pdflatex
LATEXFLAGS = --output-directory='$(BUILD)' $(LLATEXFLAGS)
PDFLATEXFLAGS = $(LATEXFLAGS) $(LPDFLATEXFLAGS)
BIBTEX = bibtex

# Directory for TeX's generated files.
BUILD = .
# BUILDD should be equivalent to $(BUILD)/
BUILDD =
VPATH = $(BUILD)

-include localdefs


==> make/commonrules <==
# Some basic recursive rules for building, installing, and cleaning up
# a source tree
#
subdirs:
	@sub="$(SUBDIRS)"; \
	for i in $$sub; do if test -n "$$i"; then \
	      (cd $$i; make); \
	fi; done;

clean:  localclean
	@sub="$(SUBDIRS)"; \
	for i in $$sub; do if test -n "$$i"; then \
	      (cd $$i; make $@); \
	fi; done;

localclean:
	$(RM) $(DIRT)

clobber: localclean
	@sub="$(SUBDIRS)";						      \
	for i in $$sub; do if test -n "$$i"; then			      \
	      (cd $$i; make $@);					      \
	fi; done;
	$(RM) $(TARGETS) $(GENERATED)

install: default localinstall
	@sub="$(SUBDIRS)";						      \
	for i in $$sub; do if test -n "$$i"; then			      \
	      (cd $$i; make $@);					      \
	fi; done;

incdepend: .dependtime
depend: .dependtime

.dependtime: $(SOURCES)
	touch temp
	$(MKDEPEND) $(MKDEPC++FLAGS) -f temp $(C++FILES)
	touch $(MKDEPFILE)
	$(MKDEPEND) $(MKDEPCFLAGS) -f $(MKDEPFILE) $(CFILES)
	cat temp >> $(MKDEPFILE)
	$(RM) temp
	touch $@

# Rules for TeX files
#
# The line that runs LATEX needs to run inside a subshell to turn off
# "make"'s status checking. It blows away .aux because the .aux file
# created is bad and also breaks bibtex. It touches .stamp to force a
# rebuild.
.tex.dvi:
	@if test -r "$*.aux";						      \
	   then cp "$(BUILDD)$*.aux" "$(BUILDD)$*.auxprev";		      \
	   else echo > "$(BUILDD)$*.auxprev";				      \
	fi
	@echo "$(LATEX) $<"
	@sh -c "$(LATEX) $< || ($(RM) $*.aux; sleep 1; touch \"$(BUILDD)$*.stamp\"; exit 1)"
	@-cmp -s "$(BUILDD)$*.aux" "$(BUILDD)$*.auxprev";		      \
	if test $$? = 1;						      \
	then								      \
	    sleep 1;							      \
	    echo "==> Rebuilding $@";					      \
	    touch "$(BUILDD)$*.stamp";					      \
	    $(MAKE) $@;							      \
	else								      \
	    echo "==> No need to rebuild $@";				      \
	fi
	@$(RM) "$(BUILDD)$*.auxprev"

.tex.pdf:
	@if test -r "$(BUILDD)$*.aux";					      \
	   then cp "$(BUILDD)$*.aux" "$(BUILDD)$*.auxprev";		      \
	   else echo > "$(BUILDD)$*.auxprev";				      \
	fi
	@echo "$(PDFLATEX) $<"
	@sh -c "$(PDFLATEX) $< || ($(RM) $*.aux; sleep 1; touch \"$(BUILDD)$*.stamp\"; exit 1)"
	@-cmp -s "$(BUILDD)$*.aux" "$(BUILDD)$*.auxprev";		      \
	if test $$? = 1;						      \
	then								      \
	    sleep 1;							      \
	    echo "==> Rebuilding $@";					      \
	    touch "$(BUILDD)$*.stamp";					      \
	    $(MAKE) $@;							      \
	else								      \
	    echo "==> No need to rebuild $@";				      \
	fi
	@$(RM) "$(BUILDD)$*.auxprev"

# must add dependencies like
#    foo.ind: foo.stamp
#    foo.dvi: foo.ind
# to use this rule properly.
.tex.ind:
	@if [ -f $*.idx ]; then						      \
	   echo makeindex $*.idx;					      \
	   makeindex $*.idx;						      \
	else								      \
	   echo touch $@;						      \
	   touch $@;							      \
        fi

# must add dependencies like
#    foo.bbl: foo.bib
#    foo.dvi: foo.bbl
# to use this rule properly.
.tex.bbl:
	@if [ -r $*.aux ]; then echo $(BIBTEX) $*; sh -c "$(BIBTEX) $* || echo"; else echo; fi

.tex.stamp: # backward compatibility
	touch $@

.dvi.ps:
	$(DVIPS) $(DVIPSOPTS) $< -o $@
.eps.pdf:
	epstopdf $(EPSTOPDFOPTS) $<

#
# Rules for C++ and .i files
#

.C.i:
	$(C++F) -E $< > $@

.c.i:
	$(CCF) -E $< > $@

.C.o:
	$(C++F) -c $<

# include $(M3SU)    # old Modula-3 rules

# Paper versions
markup:
	@DOC=markup MAKEFLAGS=e $(MAKE)
draft:
	@DOC=draft MAKEFLAGS=e $(MAKE)
tr:
	@DOC=tr MAKEFLAGS=e $(MAKE)
trdraft:
	@DOC=trdraft MAKEFLAGS=e $(MAKE)
local:
	@DOC=local MAKEFLAGS=e $(MAKE)
submission:
	@DOC=submission MAKEFLAGS=e $(MAKE)
final:
	@DOC=final MAKEFLAGS=e $(MAKE)
finaldraft:
	@DOC=finaldraft MAKEFLAGS=e $(MAKE)
blindtr:
	@DOC=blindtr MAKEFLAGS=e $(MAKE)
web:
	@DOC=web MAKEFLAGS=e $(MAKE)


==> motivation.tex <==
Existing blockchain systems have severe shortcomings in terms of
 concurrency and separation of duty.
 The goal of Charlotte is to enable efficient,
 concurrent, composable applications that rely only on their own trust
 assumptions.


==> paper.tex <==
\def\paperversion{DOC}
\def\anonymoussubmission{1} % remove or change to 0 to make submission non-anonymous
\input{paperversions}
\input{header}
\begin{document}
\input{body}
\end{document}


==> submission.tex <==
\def\paperversion{submission}
\def\anonymoussubmission{1} % remove or change to 0 to make submission non-anonymous
\input{paperversions}
\input{header}
\begin{document}
\input{body}
\end{document}


==> tex-macros/arrowsscale.tex <==
%
% this code shamelessly stolen from Andrew Stacey's answer on
% http://tex.stackexchange.com/questions/5461/is-it-possible-to-change-the-size-of-an-arrowhead-in-tikz-pgf
%

\makeatletter
\pgfkeys{
  /pgf/scalable arrows/.code={
    \let\pgf@add@arrows@as@needed=\pgf@add@scalable@arrows@as@needed
    \let\pgf@shorten@path@as@needed=\pgf@shorten@path@as@needed@for@scalable
  },
  /pgf/arrow scale factor/.initial=1,
}

\def\pgf@add@scalable@arrows@as@needed{%
  \pgfkeysgetvalue{/pgf/arrow scale factor}{\pgf@temp}%
  \let\pgf@restorelw=\pgfutil@empty
  \ifx\pgf@temp\pgfutil@empty
  \else
  \edef\pgf@restorelw{\noexpand\pgfsetlinewidth{\the\pgflinewidth}}%
  \pgfsetlinewidth{\pgf@temp\pgflinewidth}%
  \fi
  \ifx\pgf@startarrow\pgfutil@empty%
  \else%
    \pgflowlevelobj%
      {\pgftransformarrow{\pgfpointsecondonpath}{\pgfpointfirstonpath}}
      {\pgf@startarrow}%
  \fi%
  \ifx\pgf@endarrow\pgfutil@empty%
  \else%
    \pgflowlevelobj%
      {\pgftransformarrow{\pgfpointsecondlastonpath}{\pgfpointlastonpath}}
      {\pgf@endarrow}%
  \fi%
      \pgf@restorelw%
}

\def\pgf@shorten@path@as@needed@for@scalable{%
  \pgfkeysgetvalue{/pgf/arrow scale factor}{\pgf@temp}%
  \let\pgf@restorelw=\pgfutil@empty
  \ifx\pgf@temp\pgfutil@empty
  \else
  \edef\pgf@restorelw{\noexpand\pgfsetlinewidth{\the\pgflinewidth}}%
  \pgfsetlinewidth{\pgf@temp\pgflinewidth}%
  \fi
  \pgfprocesspathextractpoints{\pgf@arrowpath}%
  \let\pgf@arrow@next=\pgf@shorten@now%
  \ifx\pgf@shorten@start\pgfutil@empty%
    \ifx\pgf@shorten@end\pgfutil@empty%
      \ifdim\pgf@shorten@end@additional=0pt\relax%
        \ifdim\pgf@shorten@start@additional=0pt\relax%
          \let\pgf@arrow@next=\relax%
        \fi%
      \fi%
    \fi%
  \fi%
  \pgf@arrow@next%
  \pgf@restorelw%
}

\makeatother



==> tex-macros/paperversions.tex <==
% Sets options for different versions of a peer-reviewed paper. Cannot
% be a LaTeX package because it must often be used _before_
% \documentclass. Use as follows:
%
%   \def\paperversion{draft}
%   \def\anonymoussubmission{0} % optional. Value should be 0 or 1 if defined.
%   \input{paperversions}
%
% In addition to 'draft', the following document versions are
% supported: markup, local, submission, final, finaldraft, web, tr,
%            trdraft, blindtr
%
% markup:  internal draft for paper markup. Does not use submission
%          formatting or show comments.
% draft:   internal draft with standard layout (comments shown, blinded
%          if necessary)
% local:   version for local review (not blinded, warning re distribution)
% submission: submission for review (blinded if necessary)
% final: camera-ready (not blinded, no distribution warning)
% finaldraft: like final, but comments shown.
% web: version to post on a website. Like final, but with page
%      numbers and possibly information about where paper was published.
% tr: technical report
% trdraft: technical report with comments shown
% blindtr: technical report suitable for anonymous submission as
%     auxiliary material
%
% The following \if conditions are defined appropriately depending on
% which version is chosen:
%
\newif\ifsinglecolumn\singlecolumnfalse
\newif\ifwidemargins\widemarginsfalse
\newif\ifwarning\warningfalse
\newif\ifshowcomments\showcommentsfalse
\newif\ifblinded\blindedfalse
\newif\ifshowlinenums\showlinenumsfalse
\newif\ifreport\reportfalse
\newif\ifcopyrightspace\copyrightspacefalse
\newif\ifacknowledgments\acknowledgmentsfalse
\newif\ifshowpagenumbers\showpagenumberstrue
\newif\iffinalformat\finalformatfalse
\newif\ifweb\webfalse

% The condition \ifblinded is turned on if the file
% .blinded exists or if \anonymoussubmission is defined to be 1, unless
% overridden by the document version chosen. The local, final, tr,
% trdraft, and web versions are not blinded.
%
\ifx\anonymoussubmission\undefined
  \typeout{** Checking for .blinded file to see if venue has anonymous submission **}
\else
  \if\anonymoussubmission 1
    \blindedtrue
  \else
    \blindedfalse
  \fi
\fi
\IfFileExists{.blinded}{\blindedtrue}

\def\xxmarkup{0}
\def\xxdraft{1}
\def\xxlocal{2}
\def\xxsubmission{3}
\def\xxfinal{4}
\def\xxtr{5}
\def\xxtrdraft{6}
\def\xxfinaldraft{7}
\def\xxweb{8}
\def\xxblindtr{9}

\ifx\paperversion\xxxxundefined
\PackageError{paperversions}{*** No valid document version was specified.
Macro paperversions must be defined as one of (markup, draft,
local, submission, final, web, tr, trdraft)}
\fi

\def\xxversion{\csname xx\paperversion\endcsname}
\newif\ifsawversion\sawversionfalse

\ifcase\xxversion\relax
%markup
    \widemarginstrue
    \singlecolumntrue
    \warningtrue
    \showlinenumstrue
    \sawversiontrue
    \blindedfalse
\or %draft
    \warningtrue
    \showlinenumsfalse
    \showcommentstrue
    \sawversiontrue
\or %local
    \warningtrue
    \showcommentsfalse
    \blindedfalse
    \sawversiontrue
    \acknowledgmentstrue
    \showlinenumstrue
\or %submission
    \sawversiontrue
    \showlinenumstrue
\or %final
    \blindedfalse
    \sawversiontrue
    \copyrightspacetrue
    \acknowledgmentstrue
    \showpagenumbersfalse
    \finalformattrue
\or %tr
    \singlecolumntrue
    \blindedfalse
    \sawversiontrue
    \reporttrue
    \acknowledgmentstrue
    \webtrue
\or %trdraft
    \blindedfalse
    \singlecolumntrue
    \showcommentstrue
    \sawversiontrue
    \reporttrue
    \showlinenumstrue
    \warningtrue
\or %finaldraft
    \blindedfalse
    \showcommentstrue
    \copyrightspacetrue
    \acknowledgmentstrue
    \sawversiontrue
    \finalformattrue
    \showlinenumstrue
    \warningtrue
\or %web
    \blindedfalse
    \sawversiontrue
    \copyrightspacetrue
    \acknowledgmentstrue
    \finalformattrue
    \webtrue
\or %blindtr
    \singlecolumntrue
    \blindedtrue
    \acknowledgmentsfalse
    \sawversiontrue
    \reporttrue
    \webtrue
\fi

\ifsawversion
\else
    \typeout{*** Internal error: no valid document version processed! ***}
\fi

% Cleanup.
\let\xxmarkup=\undefined
\let\xxlocal=\undefined
\let\xxsubmission=\undefined
\let\xxfinal=\undefined
\let\xxfinaldraft=\undefined
\let\xxtr=\undefined
\let\xxtrdraft=\undefined
\let\xxweb=\undefined
\let\xxblindtr=\undefined
\let\xxversion=\undefined


==> tr.tex <==
\def\paperversion{tr}
\def\anonymoussubmission{1} % remove or change to 0 to make submission non-anonymous
\input{paperversions}
\input{header}
\begin{document}
\input{body}
\end{document}


==> trdraft.tex <==
\def\paperversion{trdraft}
\def\anonymoussubmission{1} % remove or change to 0 to make submission non-anonymous
\input{paperversions}
\input{header}
\begin{document}
\input{body}
\end{document}

